Prompt Engineering or Fine-Tuning: An Empirical Assessment of LLMs for Code

The rapid advancements in large language models (LLMs) have greatly expanded the potential for automated code-related tasks. Two primary methodologies are used in this domain: prompt engineering and fine-tuning. Prompt engineering involves applying different strategies to query LLMs, like ChatGPT, while fine-tuning further adapts pre-trained models, such as CodeBERT, by training them on task-specific data. Despite the growth in the area, there remains a lack of comprehensive comparative analysis between the approaches for code models. In this paper, we evaluate GPT-4 using three prompt engineering strategies -- basic prompting, in-context learning, and task-specific prompting -- and compare it against 17 fine-tuned models across three code-related tasks: code summarization, generation, and translation. Our results indicate that GPT-4 with prompt engineering does not consistently outperform fine-tuned models. For instance, in code generation, GPT-4 is outperformed by fine-tuned models by 28.3% points on the MBPP dataset. It also shows mixed results for code translation tasks. Additionally, a user study was conducted involving 27 graduate students and 10 industry practitioners. The study revealed that GPT-4 with conversational prompts, incorporating human feedback during interaction, significantly improved performance compared to automated prompting. Participants often provided explicit instructions or added context during these interactions. These findings suggest that GPT-4 with conversational prompting holds significant promise for automated code-related tasks, whereas fully automated prompt engineering without human involvement still requires further investigation.

==> figure/data_ex.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}

% \vspace{10pt}
\begin{minipage}{0.9\linewidth}
\begin{lstlisting}[caption={Input/output example of the tasks.},captionpos=b,label={lst:data_ex}]
### code summarization task
# input code:
def delete_database(self, database_name):
    if database_name is None:
        raise AirflowBadRequest("Database name cannot be None.")
    self.get_conn().DeleteDatabase( get_database_link(database_name))
# output summary:
'Deletes an existing database in CosmosDB.'

### code generation task
# input description:
'Write a python function to find the volume of a triangular prism.'
# output code:
def find_Volume(l,b,h):
    return ((l * b * h) / 2)

### code translation task
# Java code
public void print(String str1) {
    write(str1 != null ? str1 : String.valueOf((Object) null));}

# C# code
public virtual void print(string str1) {
    write(str1 != null ? str1 : Sharpen.StringHelper.GetValueOf((object)null));}
\end{lstlisting}
\end{minipage}
\vspace{-0.1in}

==> figure/demographics_sav.tex <==
\begin{figure*}
\centering
\resizebox{0.7\textwidth}{!}{
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=2000]{
51.9/1-3,
11.1/4-6,
7.4/6$<$,
29.6/$<$1}
\end{tikzpicture}
\caption{Student experience}
\label{fig:demo_exp}
\end{subfigure}
\hspace{0.5em}
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=230]{33.3/B,
59.3/I,
7.4/A}
\end{tikzpicture}
\caption{Student \texttt{Java} skills}
\label{fig:demo_java}
\end{subfigure}
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=130]{74.1/B,
18.5/I,
7.4/A}
\end{tikzpicture}
\caption{Student \texttt{C\#} skills}
\label{fig:demo_csharp}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=60]{
14.8/G,
37.0/VG,
33.3/E,
3.7/F,
11.1/N
}
\end{tikzpicture}
\caption{Student writing skills}
\label{fig:demo_english}
\end{subfigure}
}
%\hspace{2em}

\resizebox{0.7\textwidth}{!}{
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=190]{
30/1-3,
30/4-6,
40/6$<$}
\end{tikzpicture}
\caption{Industry experience}
\label{fig:demo_exp}
\end{subfigure}
\hspace{0.5em}
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=110]{20/B,
50/I,
30/A}
\end{tikzpicture}
\caption{Industry \texttt{Java} skills}
\label{fig:demo_java}
\end{subfigure}
\begin{subfigure}[b]{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=120]{70/B,
20/I,
10/A}
\end{tikzpicture}
\caption{Industry \texttt{C\#} skills}
\label{fig:demo_csharp}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
\centering
\begin{tikzpicture}[baseline]
\pie[scale=.51,rotate=20]{
20/G,
20/VG,
60/E}
\end{tikzpicture}
\caption{Industry writing skills}
\label{fig:demo_english}
\end{subfigure}
}

\caption{{Demographics of student (a--d) and industry (e--h) participants.} (B=Beginner, I=Intermediate, A=Advanced), (F=Fair, G=Good, VG=Very good, E=Excellent, but not native, N=Native).}
\label{fig:demographics}
\end{figure*}

==> figure/in_context_prompt.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Python,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}
% \vspace{10pt}
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={The in-context learning prompt used for quantitative analysis.},captionpos=b,label={lst:in_context_prompt}]
### code summarization task
f"Given a {lang} code snippet surrounded in ???, 
generate one line of semantic focused and abstract summarization ???{code}???"

### code generation task
f"Generate Python source code for a function, 
given a natural language prompt (surrounded by ???) describing the function's purpose.
Output only the Python source code on exactly one line. ???{nl}???"

### code translation task
f"Given that the code surrounded by ??? is written in C#, 
output only the corresponding Java code condensed on one line ???{code}???"

\end{lstlisting}
\end{minipage}

==> sections/related.tex <==
\section{Related Works}
\label{sec:related}
%\subsection{LLMs in Software Engineering}
In this section, we overview the related literature that analyzes the prompt engineering of LLMs in software engineering.
Gao et al. \cite{gao2023constructing} empirically investigated the three key factors in in-context learning in code intelligence tasks: selection, order, and number of examples. They found that both similarity and diversity in example selection are important in both performance and stability in predictions. They also find that the order and the number of examples have an impact on their performance.
Li et al. \cite{li2023nuances} investigated \emph{ChatGPT}'s ability to find correct failure-inducing test cases for buggy source code. From their initial finding, \emph{ChatGPT} had a low success rate, but after guiding it to focus with correct nuances, they were able to improve the performance drastically.
%First et al. \cite{first2023baldur} proposed a new method to automate formal verification using LLMs. They aim to generate whole proofs for theorems and combine them with a repair model to improve the generation results.
%Wei et al. \cite{wei2023copiloting} proposed \emph{Repilot}, which is a framework to copilot LLMs by synthesizing LLMs with a completion engine to generate more valid patches when doing an automated program repair task.
%Zhang et al. \cite{zhang2023multilingual} propose a novel task of translating code changes from one programming language to another using large language models (LLMs). They design and implement \emph{Codeditor}, which learns to align and apply edits across programming languages.
%Jin et al. \cite{jin2023assess} present a large-scale empirical study on how on-call engineers deal with cloud outages at Microsoft and identify the challenges and needs for outage understanding. They proposed \emph{Oasis}, a novel approach that can automatically assess the impact scope of outages and generate human-readable summaries using LLMs.
%Jin et al. \cite{jin2023inferfix} proposed \emph{InferFix}. This novel framework combines a static analyzer and an LLM to automatically fix critical security and performance bugs in Java and C\# code. They also introduced \emph{InferredBugs}, a new dataset of bugs and fixes extracted by running the \emph{Infer} static analyzer on thousands of Java and C\# repositories, with rich metadata such as bug type, location, and change history.
%Kang et al. \cite{kang2023large} proposed \emph{LIBRO}, a framework that uses LLMs to generate tests from bug reports automatically. They evaluated it on the \emph{Defects4J} benchmark and showed that it could reproduce 33\% of all studied bugs, ranking the correct test in first place for 149 bugs.
%Guo et al. \cite{guo2023exploring} conducted the first empirical study on evaluating \emph{ChatGPT}'s potential in code refinement tasks based on review comments. They created a new code review dataset with high quality and compared \emph{ChatGPT} with \emph{CodeReviewer}, a state-of-the-art code review tool.
Feng et al. \cite{feng2023prompting} proposed \emph{AdbGPT}, a novel approach that uses LLMs to automatically reproduce bugs from bug reports without any training or hard-coding effort. They designed prompts that leverage few-shot learning and chain-of-thought reasoning to elicit LLMs' knowledge and logical reasoning for bug replay.
Geng et al. \cite{geng2024large} investigated LLMs' performance in summarizing code with multiple intents regarding their properties. They adopted the in-context learning paradigm and designed customized strategies, such as selection and re-ranking techniques, to enhance performance.
%\subsection{Human-involved studies on LLMs}
%Zhai \cite{zhai2022chatgpt} explored a user-experience study on \emph{ChatGPT} where he piloted it to write an academic paper. The results showed that \emph{ChatGPT} was able to write coherently, accurately, informatively, and systematically and concluded that students should be able to learn AI tools and adjust themselves to a new learning paradigm. 
%Dwivedi et al. \cite{dwivedi2023so} listed 43 contributions of \emph{ChatGPT} in various fields, i.e., computer science, marketing, education, policy, management, etc., to investigate the opportunities and challenges of \emph{ChatGPT} in various fields. They conclude that AI tools like \emph{ChatGPT} offer a major improvement in productivity, but practitioners should also be aware of challenges, i.e., ethics, morale, privacy/security, bias, misuse, and misinformation.
%Feng et al. \cite{feng2023investigating} investigated the social media (Twitter and Reddit) on how developers use \emph{ChatGPT} for code generation tasks. They analyzed different data, i.e., the most common programming language, the purpose of use, the quality of code, the diversity of prompts, the dominant emotion associations, etc. 
%Choudhury and Shamszare \cite{choudhury2023investigating} investigated the impact of users' trust when using \emph{ChatGPT}. They surveyed 607 participants to find the correlation between users' trust and its impact on intention and actual use of the technology, and they found that trust has a direct effect on both of them.
Kabir et al. \cite{kabir2023answers} did an analysis on \emph{ChatGPT}'s responses to Stack Overflow (SO) questions to software engineering tasks. They analyzed 517 SO questions, linguistic analysis, and a user study and found more than half of the answers were incorrect, and 77\% of them were verbose. However, users still preferred \emph{ChatGPT} 39.34\% of the time due to the comprehensiveness and the style of language.
%Skjuve et al. \cite{skjuve2023user} surveyed 194 participants inquiring about their experiences with \emph{ChatGPT}.
%They found that the majority of users have a positive experience with its usefulness in practical responses and its creative outcomes.
%Amaro et al. \cite{amaro2023ai} investigated the reliability of \emph{ChatGPT}'s responses and how experts perceive them. They conducted a user study on 15 participants and showed a set of queries and their correct and incorrect answers from the model. Even though the participants knew the model generated incorrect answers, they were positive about using them, indicating the importance of verification and interpretation of human evaluators.


